Jupiter and Saturn as Spectral Analogs for Extrasolar Gas Giants and Brown Dwarfs

With the advent of direct imaging spectroscopy, the number of spectra from brown dwarfs and extrasolar gas giants is growing rapidly. Many brown dwarfs and extrasolar gas giants exhibit spectroscopic and photometric variability, which is likely the result of weather patterns. However, for the foreseeable future, point-source observations will be the only viable method to extract brown dwarf and exoplanet spectra. Models have been able to reproduce the observed variability, but ground truth observations are required to verify their results. To that end, we provide visual and near-infrared spectra of Jupiter and Saturn obtained from the \emph{Cassini} VIMS instrument. We disk-integrate the VIMS spectral cubes to simulate the spectra of Jupiter and Saturn as if they were directly imaged exoplanets or brown dwarfs. We present six empirical disk-integrated spectra for both Jupiter and Saturn with phase coverage of $1.7^\circ$ to $133.5^\circ$ and $39.6^\circ$ to $110.2^\circ$, respectively. To understand the constituents of these disk-integrated spectra, we also provide end member (single feature) spectra for permutations of illumination and cloud density, as well as for Saturn's rings. In tandem, these disk-integrated and end member spectra provide the ground truth needed to analyze point source spectra from extrasolar gas giants and brown dwarfs. Lastly, we discuss the impact that icy rings, such as Saturn's, have on disk-integrated spectra and consider the feasibility of inferring the presence of rings from direct imaging spectra.

==> references.tex <==
@article{Acton_1999,
  title={in Lunar and Planetary Science Conference},
  author={{Acton}, C. H.},
  journal={Lunar and Planetary Science Conference},
  year={1999},
}

@article{Apai_2013,
  title={HST spectral mapping of L/T transition brown dwarfs reveals cloud thickness variations},
  author={Apai, D{\'a}niel and Radigan, Jacqueline and Buenzli, Esther and Burrows, Adam and Reid, Iain Neill and Jayawardhana, Ray},
  journal={The Astrophysical Journal},
  volume={768},
  number={2},
  pages={121},
  year={2013},
  publisher={IOP Publishing}
}

@misc{Apai_2017,
      title={Exploring Other Worlds: Science Questions for Future Direct Imaging Missions (EXOPAG SAG15 Report)}, 
      author={Daniel Apai and Nicolas Cowan and Ravikumar Kopparapu and Markus Kasper and Renyu Hu and Caroline Morley and Yuka Fujii and Stephen Kane and Mark Maley and Anthony del Genio and Theodora Karalidi and Thaddeus Komacek and Eric Mamajek and Avi Mandell and Shawn Domagal-Goldman and Travis Barman and Alan Boss and James Breckinridge and Ian Crossfield and William Danchi and Eric Ford and Nicolas Iro and James Kasting and Patrick Lowrance and Nikku Madhusudhan and Michael McElwain and William Moore and Ilaria Pascucci and Peter Plavchan and Aki Roberge and Glenn Schneider and Adam Showman and Margaret Turnbull},
      year={2017},
      archivePrefix={arXiv},
      primaryClass={astro-ph.EP}
}

@article{Arnold_2004,
  title={The detectability of extrasolar planet surroundings-I. Reflected-light photometry of unresolved rings},
  author={Arnold, Luc and Schneider, Jean},
  journal={Astronomy \& Astrophysics},
  volume={420},
  number={3},
  pages={1153--1162},
  year={2004},
  publisher={EDP Sciences}
}

@article{Aumann_1969,
  title={The internal powers and effective temperatures of Jupiter and Saturn},
  author={Aumann, HH and Gillespie Jr, CM and Low, FJ},
  journal={The Astrophysical Journal},
  volume={157},
  pages={L69},
  year={1969}
}

@article{Baines_2005,
  title={THE ATMOSPHERES OF SATURN AND TITAN IN THE NEAR-INFRARED: FIRST RESULTS OF CASSINI/VIMS},
  author={{Baines}, K. H. and P. Drossart and T. W. Momary and V. FORMISANO and C. GRIFFITH and G. BELLUCCI and J. P. BIBRING and R. H. BROWN and B. J. BURATTI and F. CAPACCIONI and P. CERRONI and R. N. CLARK and A. CORADINI and M. COMBES and D. P. CRUIKSHANK and R. JAUMANN and Y. LANGEVIN and D. L. MATSON and T. B. MCCORD and V. MENNELLA and R. M. NELSON and P. D. NICHOLSON and B. SICARDY and C. SOTIN },
  journal={Earth, Moon, and Planets},
  volume={96},
  pages={119--147},
  year={2005},
  publisher={Springer}
}

@article{Barnes_2007,
  title={Global-scale surface spectral variations on Titan seen from Cassini/VIMS},
  author={{Barnes}, Jason W and Brown, Robert H and Soderblom, Laurence and Buratti, Bonnie J and Sotin, Christophe and Rodriguez, Sebastien and Le Mou{\`e}lic, Stephane and Baines, Kevin H and Clark, Roger and Nicholson, Phil},
  journal={Icarus},
  volume={186},
  number={1},
  pages={242--258},
  year={2007},
  publisher={Elsevier}
}

@article{Biller_2017,
  title={The time domain for brown dwarfs and directly imaged giant exoplanets: the power of variability monitoring},
  author={Biller, Beth},
  journal={Astronomical Review},
  volume={13},
  number={1},
  pages={1--27},
  year={2017},
  publisher={Taylor \& Francis}
}

@article{Biller_2018,
  title={Exoplanet atmosphere measurements from direct imaging},
  author={Biller, Beth A and Bonnefoy, Micka{\"e}l},
  journal={arXiv preprint arXiv:1807.05136},
  year={2018}
}

@article{Brown_2004,
  title={The Cassini visual and infrared mapping spectrometer (VIMS) investigation},
  author={{Brown}, Robert H and Baines, Kevin H and Bellucci, Gꎬ and Bibring, J-P and Buratti, Bonnie J and Capaccioni, F and Cerroni, P and Clark, Roger N and Coradini, Angioletta and Cruikshank, Dale P and others},
  journal={Space Science Reviews},
  volume={115},
  number={1-4},
  pages={111--168},
  year={2004},
  publisher={Springer}
}

@article{Burgasser_2002a,
  title={The spectra of T dwarfs. I. Near-infrared data and spectral classification},
  author={{Burgasser}, Adam J and Kirkpatrick, J Davy and Brown, Michael E and Reid, I Neill and Burrows, Adam and Liebert, James and Matthews, Keith and Gizis, John E and Dahn, Conard C and Monet, David G and others},
  journal={\apj},
  volume={564},
  number={1},
  pages={421},
  year={2002},
  publisher={IOP Publishing}
}

@article{Burgasser_2002b,
  title={Evidence of cloud disruption in the L/T dwarf transition},
  author={Burgasser, Adam J and Marley, Mark S and Ackerman, Andrew S and Saumon, Didier and Lodders, Katharina and Dahn, Conard C and Harris, Hugh C and Kirkpatrick, J Davy},
  journal={The Astrophysical Journal},
  volume={571},
  number={2},
  pages={L151},
  year={2002},
  publisher={IOP Publishing}
}

@article{Crossfield_2014a,
  title={A global cloud map of the nearest known brown dwarf},
  author={{Crossfield}, IJM and Biller, B and Schlieder, JE and Deacon, NR and Bonnefoy, M and Homeier, D and Allard, F and Buenzli, E and Henning, Th and Brandner, W and others},
  journal={Nature},
  volume={505},
  number={7485},
  pages={654--656},
  year={2014},
  publisher={Nature Publishing Group}
}

@article{Crossfield_2014b,
  title={Doppler imaging of exoplanets and brown dwarfs},
  author={{Crossfield}, Ian JM},
  journal={Astronomy \& Astrophysics},
  volume={566},
  pages={A130},
  year={2014},
  publisher={EDP Sciences}
}

@article{Cushing_2011,
  title={The discovery of Y dwarfs using data from the wide-field infrared survey explorer (WISE)},
  author={{Cushing}, Michael C and Kirkpatrick, J Davy and Gelino, Christopher R and Griffith, Roger L and Skrutskie, Michael F and Mainzer, A and Marsh, Kenneth A and Beichman, Charles A and Burgasser, Adam J and Prato, Lisa A and others},
  journal={\apj},
  volume={743},
  number={1},
  pages={50},
  year={2011},
  publisher={IOP Publishing}
}

@article{Cushing_2016,
  title={THE FIRST DETECTION OF PHOTOMETRIC VARIABILITY IN AY DWARF: WISE J140518. 39+ 553421.3},
  author={Cushing, Michael C and Hardegree-Ullman, Kevin K and Trucks, Jesica L and Morley, Caroline V and Gizis, John E and Marley, Mark S and Fortney, Jonathan J and Kirkpatrick, J Davy and Gelino, Christopher R and Mace, Gregory N and others},
  journal={The Astrophysical Journal},
  volume={823},
  number={2},
  pages={152},
  year={2016},
  publisher={IOP Publishing}
}

@article{Damiano_2020a,
  title={Multi-orbital-phase and multiband characterization of exoplanetary atmospheres with reflected light spectra},
  author={Damiano, Mario and Hu, Renyu and Hildebrandt, Sergi R},
  journal={The Astronomical Journal},
  volume={160},
  number={5},
  pages={206},
  year={2020},
  publisher={IOP Publishing}
}

@article{Damiano_2020b,
  title={Exorel: a Bayesian inverse retrieval framework for exoplanetary reflected light spectra},
  author={Damiano, Mario and Hu, Renyu},
  journal={The Astronomical Journal},
  volume={159},
  number={4},
  pages={175},
  year={2020},
  publisher={IOP Publishing}
}

@BOOK{Decadal_2020,  author    = "{National Academies of Sciences, Engineering, and Medicine}",  title     = "Pathways to Discovery in Astronomy and Astrophysics for the 2020s",  isbn      = "978-0-309-46586-1",
  year      =2021,
  publisher = "The National Academies Press",
}

@article{Dyudina_2005,
  title={Phase light curves for extrasolar Jupiters and Saturns},
  author={Dyudina, Ulyana A and Sackett, Penny D and Bayliss, Daniel DR and Seager, Sara and Porco, Carolyn C and Throop, Henry B and Dones, Luke},
  journal={The Astrophysical Journal},
  volume={618},
  number={2},
  pages={973},
  year={2005},
  publisher={IOP Publishing}
}

@article{Fortney_2020,
  title={Beyond Equilibrium Temperature: How the Atmosphere/Interior Connection Affects the Onset of Methane, Ammonia, and Clouds in Warm Transiting Giant Planets},
  author={Fortney, Jonathan J and Visscher, Channon and Marley, Mark S and Hood, Callie E and Line, Michael R and Thorngren, Daniel P and Freedman, Richard S and Lupu, Roxana},
  journal={The Astronomical Journal},
  volume={160},
  number={6},
  pages={288},
  year={2020},
  publisher={IOP Publishing}
}

@article{Ge_2019,
  title={Rotational light curves of Jupiter from ultraviolet to mid-infrared and implications for brown dwarfs and exoplanets},
  author={Ge, Huazhi and Zhang, Xi and Fletcher, Leigh N and Orton, Glenn S and Sinclair, James and Fernandes, Josh and Momary, Tom and Kasaba, Yasumasa and Sato, Takao M and Fujiyoshi, Takuya},
  journal={The Astronomical Journal},
  volume={157},
  number={2},
  pages={89},
  year={2019},
  publisher={IOP Publishing}
}

@inproceedings{Gelino_2000,
  title={Variability in an unresolved Jupiter},
  author={Gelino, C and Marley, M},
  booktitle={From Giant Planets to Cool Stars},
  volume={212},
  pages={322},
  year={2000}
}

@article{Gu_2021,
  title={Earth as a Proxy Exoplanet: Deconstructing and Reconstructing Spectrophotometric Light Curves},
  author={Gu, Lixiang and Fan, Siteng and Li, Jiazheng and Bartlett, Stuart J and Natraj, Vijay and Jiang, Jonathan H and Crisp, David and Hu, Yongyun and Tinetti, Giovanna and Yung, Yuk L},
  journal={The Astronomical Journal},
  volume={161},
  number={3},
  pages={122},
  year={2021},
  publisher={IOP Publishing}
}

@article{Heng_2021,
  title={Jupiter as an exoplanet: insights from Cassini phase curves},
  author={Heng, Kevin and Li, Liming},
  journal={The Astrophysical Journal Letters},
  volume={909},
  number={2},
  pages={L20},
  year={2021},
  publisher={IOP Publishing}
}

@article{Jiang_2018,
  title={Using deep space climate observatory measurements to study the Earth as an exoplanet},
  author={Jiang, Jonathan H and Zhai, Albert J and Herman, Jay and Zhai, Chengxing and Hu, Renyu and Su, Hui and Natraj, Vijay and Li, Jiazheng and Xu, Feng and Yung, Yuk L},
  journal={The Astronomical Journal},
  volume={156},
  number={1},
  pages={26},
  year={2018},
  publisher={IOP Publishing}
}

@article{Kirkpatrick_1999,
  title={Dwarfs cooler than “M”: The definition of spectral type “L” using discoveries from the 2-Micron All-Sky Survey (2MASS)},
  author={{Kirkpatrick}, J. Davy and Reid, I Neill and Liebert, James and Cutri, Roc M and Nelson, Brant and Beichman, Charles A and Dahn, Conard C and Monet, David G and Gizis, John E and Skrutskie, Michael F},
  journal={\apj},
  volume={519},
  number={2},
  pages={802},
  year={1999},
  publisher={IOP Publishing}
}

@article{Leggett_2015,
  title={Near-infrared photometry of Y dwarfs: low ammonia abundance and the onset of water clouds},
  author={Leggett, SK and Morley, Caroline V and Marley, MS and Saumon, D},
  journal={The Astrophysical Journal},
  volume={799},
  number={1},
  pages={37},
  year={2015},
  publisher={IOP Publishing}
}

@article{Leggett_2016,
  title={Near-infrared spectroscopy of the Y0 WISEP J173835. 52+ 273258.9 and the Y1 WISE J035000. 32--565830.2: The importance of non-equilibrium chemistry},
  author={Leggett, Sandy K and Tremblin, Patrick and Saumon, Didier and Marley, Mark S and Morley, Caroline V and Amundsen, David S and Baraffe, Isabelle and Chabrier, Gilles},
  journal={The Astrophysical Journal},
  volume={824},
  number={1},
  pages={2},
  year={2016},
  publisher={IOP Publishing}
}

@article{Lew_2020,
  title={Cloud Atlas: Unraveling the vertical cloud structure with the time-series spectrophotometry of an unusually red brown dwarf},
  author={Lew, Ben WP and Apai, D{\'a}niel and Marley, Mark and Saumon, Didier and Schneider, Glenn and Zhou, Yifan and Cowan, Nicolas B and Karalidi, Theodora and Manjavacas, Elena and Bedin, LR and others},
  journal={The Astrophysical Journal},
  volume={903},
  number={1},
  pages={15},
  year={2020},
  publisher={IOP Publishing}
}

@article{Livengood_2011,
  title={Properties of an Earth-like planet orbiting a Sun-like star: Earth observed by the EPOXI mission},
  author={Livengood, Timothy A and Deming, L Drake and A'hearn, Michael F and Charbonneau, David and Hewagama, Tilak and Lisse, Carey M and McFadden, Lucy A and Meadows, Victoria S and Robinson, Tyler D and Seager, Sara and others},
  journal={Astrobiology},
  volume={11},
  number={9},
  pages={907--930},
  year={2011},
  publisher={Mary Ann Liebert, Inc. 140 Huguenot Street, 3rd Floor New Rochelle, NY 10801 USA}
}

@article{Luhman_2014,
  title={Discovery of a~ 250 K brown dwarf at 2 pc from the sun},
  author={{Luhman}, K. L.},
  journal={\apjl},
  volume={786},
  number={2},
  pages={L18},
  year={2014},
  publisher={IOP Publishing}
}

@article{Lupu_2016,
  title={Developing atmospheric retrieval methods for direct imaging spectroscopy of gas giants in reflected light. I. Methane abundances and basic cloud properties},
  author={Lupu, Roxana E and Marley, Mark S and Lewis, Nikole and Line, Michael and Traub, Wesley A and Zahnle, Kevin},
  journal={The Astronomical Journal},
  volume={152},
  number={6},
  pages={217},
  year={2016},
  publisher={IOP Publishing}
}

@article{Macdonald_2018,
  title={Exploring H2O prominence in reflection spectra of cool giant planets},
  author={MacDonald, Ryan J and Marley, Mark S and Fortney, Jonathan J and Lewis, Nikole K},
  journal={The Astrophysical Journal},
  volume={858},
  number={2},
  pages={69},
  year={2018},
  publisher={IOP Publishing}
}

@article{Marley_1999,
  title={Reflected spectra and albedos of extrasolar giant planets. I. Clear and cloudy atmospheres},
  author={Marley, Mark S and Gelino, Christopher and Stephens, Denise and Lunine, Jonathan I and Freedman, Richard},
  journal={The Astrophysical Journal},
  volume={513},
  number={2},
  pages={879},
  year={1999},
  publisher={IOP Publishing}
}

@article{Marley_2010,
  title={A patchy cloud model for the L to T dwarf transition},
  author={{Marley}, Mark S and Saumon, Didier and Goldblatt, Colin},
  journal={\apjl},
  volume={723},
  number={1},
  pages={L117},
  year={2010},
  publisher={IOP Publishing}
}

@article{Marley_2014,
  title={On the cool side: modeling the atmospheres of brown dwarfs and giant planets},
  author={Marley, Mark S and Robinson, Tyler D},
  journal={arXiv preprint arXiv:1410.6512},
  year={2014}
}

@article{Martin_2020,
  title={The Planet as Exoplanet Analog Spectrograph (PEAS): design and first-light},
  author={Martin, Emily C and Skemer, Andrew J and Radovan, Matthew V and Allen, Steven L and Black, David and Deich, William TS and Fortney, Jonathan J and Kruglikov, Gabriel and MacDonald, Nicholas and Marques, David and others},
  booktitle={Ground-based and Airborne Instrumentation for Astronomy VIII},
  volume={11447},
  pages={135--143},
  year={2020},
  organization={SPIE}
}

@article{Mayorga_2016,
  title={Jupiter’s phase variations from Cassini: a testbed for future direct-imaging missions},
  author={Mayorga, LC and Jackiewicz, Jason and Rages, Kathy and West, Robert A and Knowles, Ben and Lewis, N and Marley, Mark S},
  journal={The Astronomical Journal},
  volume={152},
  number={6},
  pages={209},
  year={2016},
  publisher={IOP Publishing}
}

@article{Metchev_2015,
  title={Weather on other worlds. II. Survey results: Spots are ubiquitous on L and T dwarfs},
  author={{Metchev}, Stanimir A and Heinze, Aren and Apai, D{\'a}niel and Flateau, Davin and Radigan, Jacqueline and Burgasser, Adam and Marley, Mark S and Artigau, {\'E}tienne and Plavchan, Peter and Goldman, Bertrand},
  journal={The Astrophysical Journal},
  volume={799},
  number={2},
  pages={154},
  year={2015},
  publisher={IOP Publishing}
}

@article{Morley_2018,
  title={An L band spectrum of the coldest brown dwarf},
  author={Morley, Caroline V and Skemer, Andrew J and Allers, Katelyn N and Marley, Mark S and Faherty, Jacqueline K and Visscher, Channon and Beiler, Samuel A and Miles, Brittany E and Lupu, Roxana and Freedman, Richard S and others},
  journal={The Astrophysical Journal},
  volume={858},
  number={2},
  pages={97},
  year={2018},
  publisher={IOP Publishing}
}

@article{Nayak_2017,
  title={Atmospheric retrieval for direct imaging spectroscopy of gas giants in reflected light. II. Orbital phase and planetary radius},
  author={Nayak, Michael and Lupu, Roxana and Marley, Mark S and Fortney, Jonathan J and Robinson, Tyler and Lewis, Nikole},
  journal={Publications of the Astronomical Society of the Pacific},
  volume={129},
  number={973},
  pages={034401},
  year={2017},
  publisher={IOP Publishing}
}

@article{Perez_2016,
  title={Saturn’s tropospheric particles phase function and spatial distribution from Cassini ISS 2010--11 observations},
  author={P{\'e}rez-Hoyos, Santiago and Sanz-Requena, Jos{\'e} Francisco and S{\'a}nchez-Lavega, Agust{\'\i}n and Irwin, Patrick GJ and Smith, Andrew},
  journal={Icarus},
  volume={277},
  pages={1--18},
  year={2016},
  publisher={Elsevier}
}

@article{Simon_2016,
  title={Neptune’s dynamic atmosphere from Kepler K2 observations: implications for brown dwarf light curve analyses},
  author={Simon, Amy A and Rowe, Jason F and Gaulme, Patrick and Hammel, Heidi B and Casewell, Sarah L and Fortney, Jonathan J and Gizis, John E and Lissauer, Jack J and Morales-Juberias, Raul and Orton, Glenn S and others},
  journal={The Astrophysical Journal},
  volume={817},
  number={2},
  pages={162},
  year={2016},
  publisher={IOP Publishing}
}

@article{Skemer_2016,
  title={The first spectrum of the coldest brown dwarf},
  author={Skemer, Andrew J and Morley, Caroline V and Allers, Katelyn N and Geballe, Thomas R and Marley, Mark S and Fortney, Jonathan J and Faherty, Jacqueline K and Bjoraker, Gordon L and Lupu, Roxana},
  journal={The Astrophysical Journal Letters},
  volume={826},
  number={2},
  pages={L17},
  year={2016},
  publisher={IOP Publishing}
}

@article{Sudarsky_2000,
  title={Albedo and reflection spectra of extrasolar giant planets},
  author={Sudarsky, David and Burrows, Adam and Pinto, Philip},
  journal={The Astrophysical Journal},
  volume={538},
  number={2},
  pages={885},
  year={2000},
  publisher={IOP Publishing}
}

@article{Sudarsky_2003,
  title={Theoretical spectra and atmospheres of extrasolar giant planets},
  author={Sudarsky, David and Burrows, Adam and Hubeny, Ivan},
  journal={The Astrophysical Journal},
  volume={588},
  number={2},
  pages={1121},
  year={2003},
  publisher={IOP Publishing}
}

@article{Tan_2019,
  title={Atmospheric variability driven by radiative cloud feedback in brown dwarfs and directly imaged extrasolar giant planets},
  author={Tan, Xianyu and Showman, Adam P},
  journal={The Astrophysical Journal},
  volume={874},
  number={2},
  pages={111},
  year={2019},
  publisher={IOP Publishing}
}

@article{Tan_2021,
  title={Atmospheric circulation of brown dwarfs and directly imaged exoplanets driven by cloud radiative feedback: effects of rotation},
  author={Tan, Xianyu and Showman, Adam P},
  journal={Monthly Notices of the Royal Astronomical Society},
  volume={502},
  number={1},
  pages={678--699},
  year={2021},
  publisher={Oxford University Press}
}

@article{Tomasko_1980,
  title={Photometry of Saturn at large phase angles},
  author={Tomasko, MG and McMillan, RS and Doose, LR and Castillo, ND and Dilley, JP},
  journal={Journal of Geophysical Research: Space Physics},
  volume={85},
  number={A11},
  pages={5891--5903},
  year={1980},
  publisher={Wiley Online Library}
}

@article{Traub_2010,
  title={Direct imaging of exoplanets},
  author={{Traub}, Wesley A and Oppenheimer, Ben R},
  journal={Exoplanets},
  pages={111--156},
  year={2010},
  publisher={University of Arizona Press, Tucson}
}

@article{Vdovichenko_2021,
  title={Zonal Features in the Behavior of Weak Molecular Absorption Bands on Jupiter},
  author={{Vdovichenko}, V. D. and A. M. Karimov and G. A. Kirienko and P. G. Lysenko and V. G. Tejfel and V. A. Filippov and G. A. Kharitonova and A. P. Khozhenets},
  journal={Solar System Research},
  volume={55},
  pages={35--46},
  year={2021},
  publisher={Springer}
}

@article{Yang_2016,
  title={Extrasolar storms: Pressure-dependent changes in light-curve phase in brown dwarfs from simultaneous HST and Spitzer observations},
  author={Yang, Hao and Apai, D{\'a}niel and Marley, Mark S and Karalidi, Theodora and Flateau, Davin and Showman, Adam P and Metchev, Stanimir and Buenzli, Esther and Radigan, Jacqueline and Artigau, {\'E}tienne and others},
  journal={The Astrophysical Journal},
  volume={826},
  number={1},
  pages={8},
  year={2016},
  publisher={IOP Publishing}
}

@article{Zhang_2014,
  title={Atmospheric circulation of brown dwarfs: jets, vortices, and time variability},
  author={Zhang, Xi and Showman, Adam P},
  journal={The Astrophysical Journal Letters},
  volume={788},
  number={1},
  pages={L6},
  year={2014},
  publisher={IOP Publishing}
}

@article{Zhang_2020,
  title={Atmospheric regimes and trends on exoplanets and brown dwarfs},
  author={Zhang, Xi},
  journal={Research in Astronomy and Astrophysics},
  volume={20},
  number={7},
  pages={099},
  year={2020},
  publisher={IOP Publishing}
}

@article{Zhou_2016,
  title={Discovery of rotational modulations in the planetary-mass companion 2M1207b: intermediate rotation period and heterogeneous clouds in a low gravity atmosphere},
  author={Zhou, Yifan and Apai, D{\'a}niel and Schneider, Glenn H and Marley, Mark S and Showman, Adam P},
  journal={The Astrophysical Journal},
  volume={818},
  number={2},
  pages={176},
  year={2016},
  publisher={IOP Publishing}
}


@ARTICLE{2013A&A...558A..33A,
       author = {{Astropy Collaboration} and {Robitaille}, Thomas P. and
         {Tollerud}, Erik J. and {Greenfield}, Perry and {Droettboom}, Michael and
         {Bray}, Erik and {Aldcroft}, Tom and {Davis}, Matt and
         {Ginsburg}, Adam and {Price-Whelan}, Adrian M. and
         {Kerzendorf}, Wolfgang E. and {Conley}, Alexander and {Crighton}, Neil and
         {Barbary}, Kyle and {Muna}, Demitri and {Ferguson}, Henry and
         {Grollier}, Fr{\'e}d{\'e}ric and {Parikh}, Madhura M. and
         {Nair}, Prasanth H. and {Unther}, Hans M. and {Deil}, Christoph and
         {Woillez}, Julien and {Conseil}, Simon and {Kramer}, Roban and
         {Turner}, James E.~H. and {Singer}, Leo and {Fox}, Ryan and
         {Weaver}, Benjamin A. and {Zabalza}, Victor and {Edwards}, Zachary I. and
         {Azalee Bostroem}, K. and {Burke}, D.~J. and {Casey}, Andrew R. and
         {Crawford}, Steven M. and {Dencheva}, Nadia and {Ely}, Justin and
         {Jenness}, Tim and {Labrie}, Kathleen and {Lim}, Pey Lian and
         {Pierfederici}, Francesco and {Pontzen}, Andrew and {Ptak}, Andy and
         {Refsdal}, Brian and {Servillat}, Mathieu and {Streicher}, Ole},
        title = "{Astropy: A community Python package for astronomy}",
      journal = {\aap},
     keywords = {methods: data analysis, methods: miscellaneous, virtual observatory tools, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2013",
        month = "Oct",
       volume = {558},
          eid = {A33},
        pages = {A33},
          doi = {10.1051/0004-6361/201322068},
archivePrefix = {arXiv},
       eprint = {1307.6212},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...558A..33A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996A&AS..117..393B,
       author = {{Bertin}, E. and {Arnouts}, S.},
        title = "{SExtractor: Software for source extraction.}",
      journal = {\aaps},
     keywords = {METHODS: DATA ANALYSIS, TECHNIQUES: IMAGE PROCESSING, GALAXIES: PHOTOMETRY},
         year = "1996",
        month = "Jun",
       volume = {117},
        pages = {393-404},
          doi = {10.1051/aas:1996164},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&AS..117..393B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018AJ....156...82C,
       author = {{Cloutier}, Ryan and {Doyon}, Ren{\'e} and {Bouchy}, Francois and
         {H{\'e}brard}, Guillaume},
        title = "{Quantifying the Observational Effort Required for the Radial Velocity Characterization of TESS Planets}",
      journal = {\aj},
     keywords = {methods: analytical, planets and satellites: detection, planets and satellites: fundamental parameters, techniques: radial velocities, Astrophysics - Earth and Planetary Astrophysics},
         year = "2018",
        month = "Aug",
       volume = {156},
       number = {2},
          eid = {82},
        pages = {82},
          doi = {10.3847/1538-3881/aacea9},
archivePrefix = {arXiv},
       eprint = {1807.01263},
 primaryClass = {astro-ph.EP},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....156...82C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015ApJ...805...23C,
       author = {{Corrales}, Lia},
        title = "{X-Ray Scattering Echoes and Ghost Halos from the Intergalactic Medium: Relation to the Nature of AGN Variability}",
      journal = {\apj},
     keywords = {accretion, accretion disks, dust, extinction, quasars: general, intergalactic medium, X-rays: ISM, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies},
         year = "2015",
        month = "May",
       volume = {805},
       number = {1},
          eid = {23},
        pages = {23},
          doi = {10.1088/0004-637X/805/1/23},
archivePrefix = {arXiv},
       eprint = {1503.01475},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...805...23C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013RMxAA..49..137F,
       author = {{Ferland}, G.~J. and {Porter}, R.~L. and {van Hoof}, P.~A.~M. and
         {Williams}, R.~J.~R. and {Abel}, N.~P. and {Lykins}, M.~L. and
         {Shaw}, G. and {Henney}, W.~J. and {Stancil}, P.~C.},
        title = "{The 2013 Release of Cloudy}",
      journal = {\rmxaa},
     keywords = {atomic processes, galaxies: active, methods: numerical, molecular processes, radiation mechanisms: general, Astrophysics - Galaxy Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2013",
        month = "Apr",
       volume = {49},
        pages = {137-163},
archivePrefix = {arXiv},
       eprint = {1302.4485},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013RMxAA..49..137F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1989BAAS...21..780H,
       author = {{Hanisch}, R.~J. and {Biemesderfer}, C.~D.},
        title = "{T$_{E}$X and LAT$_{E}$X Macro Definition Files for Astronomical Publications}",
    booktitle = {\baas},
         year = "1989",
        month = "Mar",
        pages = {780},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1989BAAS...21..780H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{lamport94,
       author = {{Lamport}, L.},
        title = "{LaTeX: A Document Preparation System}",
    publisher = {Addison-Wesley Professional},
	 year = "1994",
      edition = {2},
	 isbn = {0201529831}
}

@ARTICLE{2018ApJ...868L..33L,
       author = {{Li}, Leping and {Zhang}, Jun and {Peter}, Hardi and
         {Chitta}, Lakshmi Pradeep and {Su}, Jiangtao and {Song}, Hongqiang and
         {Xia}, Chun and {Hou}, Yijun},
        title = "{Quasi-periodic Fast Propagating Magnetoacoustic Waves during the Magnetic Reconnection Between Solar Coronal Loops}",
      journal = {\apj},
     keywords = {magnetic reconnection, plasmas, Sun: corona, Sun: UV radiation, waves, Astrophysics - Solar and Stellar Astrophysics},
         year = "2018",
        month = "Dec",
       volume = {868},
       number = {2},
          eid = {L33},
        pages = {L33},
          doi = {10.3847/2041-8213/aaf167},
archivePrefix = {arXiv},
       eprint = {1811.08553},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...868L..33L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016AJ....152...41P,
       author = {{Pr{\v{s}}a}, Andrej and {Harmanec}, Petr and {Torres}, Guillermo and
         {Mamajek}, Eric and {Asplund}, Martin and {Capitaine}, Nicole and
         {Christensen-Dalsgaard}, J{\o}rgen and {Depagne}, {\'E}ric and
         {Haberreiter}, Margit and {Hekker}, Saskia},
        title = "{Nominal Values for Selected Solar and Planetary Quantities: IAU 2015 Resolution B3}",
      journal = {\aj},
     keywords = {planets and satellites: fundamental parameters, standards, stars: fundamental parameters, stars: general, Sun: fundamental parameters, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2016",
        month = "Aug",
       volume = {152},
       number = {2},
          eid = {41},
        pages = {41},
          doi = {10.3847/0004-6256/152/2/41},
archivePrefix = {arXiv},
       eprint = {1605.09788},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016AJ....152...41P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJS..197...31S,
       author = {{Schwarz}, Greg J. and {Ness}, Jan-Uwe and {Osborne}, J.~P. and
         {Page}, K.~L. and {Evans}, P.~A. and {Beardmore}, A.~P. and
         {Walter}, Frederick M. and {Helton}, L. Andrew and
         {Woodward}, Charles E. and {Bode}, Mike and {Starrfield}, Sumner and
         {Drake}, Jeremy J.},
        title = "{Swift X-Ray Observations of Classical Novae. II. The Super Soft Source Sample}",
      journal = {\apjs},
     keywords = {novae, cataclysmic variables, ultraviolet: stars, X-rays: stars, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2011",
        month = "Dec",
       volume = {197},
       number = {2},
          eid = {31},
        pages = {31},
          doi = {10.1088/0067-0049/197/2/31},
archivePrefix = {arXiv},
       eprint = {1110.6224},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJS..197...31S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...793..127V,
       author = {{Vogt}, Fr{\'e}d{\'e}ric P.~A. and {Dopita}, Michael A. and
         {Kewley}, Lisa J. and {Sutherland}, Ralph S. and
         {Scharw{\"a}chter}, Julia and {Basurah}, Hassan M. and {Ali}, Alaa and
         {Amer}, Morsi A.},
        title = "{Galaxy Emission Line Classification Using Three-dimensional Line Ratio Diagrams}",
      journal = {\apj},
     keywords = {galaxies: abundances, galaxies: general, galaxies: Seyfert, galaxies: starburst, H II regions, ISM: lines and bands, Astrophysics - Astrophysics of Galaxies},
         year = "2014",
        month = "Oct",
       volume = {793},
       number = {2},
          eid = {127},
        pages = {127},
          doi = {10.1088/0004-637X/793/2/127},
archivePrefix = {arXiv},
       eprint = {1406.5186},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...793..127V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJ...777..161B,
       author = {{Barnes}, Jason W. and {Clark}, Roger N. and {Sotin}, Christophe and {{\'A}d{\'a}mkovics}, M{\'a}t{\'e} and {App{\'e}r{\'e}}, Thomas and {Rodriguez}, Sebastien and {Soderblom}, Jason M. and {Brown}, Robert H. and {Buratti}, Bonnie J. and {Baines}, Kevin H. and {Le Mou{\'e}lic}, St{\'e}phane and {Nicholson}, Philip D.},
        title = "{A Transmission Spectrum of Titan's North Polar Atmosphere from a Specular Reflection of the Sun}",
      journal = {\apj},
     keywords = {planets and satellites: individual: Titan, radiative transfer, techniques: spectroscopic},
         year = 2013,
        month = nov,
       volume = {777},
       number = {2},
          eid = {161},
        pages = {161},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...777..161B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


